Coordination of multiple mobile manipulators for ordered sorting of cluttered objects

We present a coordination method for multiple mobile manipulators to sort objects in clutter. We consider the object rearrangement problem in which the objects must be sorted into different groups in a particular order. In clutter, the order constraints could not be easily satisfied since some objects occlude other objects so the occluded ones are not directly accessible to the robots. Those objects occluding others need to be moved more than once to make the occluded objects accessible. Such rearrangement problems fall into the class of nonmonotone rearrangement problems which are computationally intractable. While the nonmonotone problems with order constraints are harder, involving with multiple robots requires another computation for task allocation. The proposed method first finds a sequence of objects to be sorted using a search such that the order constraint in each group is satisfied. The search can solve nonmonotone instances that require temporal relocation of some objects to access the next object to be sorted. Once a complete sorting sequence is found, the objects in the sequence are assigned to multiple mobile manipulators using a greedy allocation method. We develop four versions of the method with different search strategies. In the experiments, we show that our method can find a sorting sequence quickly (e.g., 4.6 sec with 20 objects sorted into five groups) even though the solved instances include hard nonmonotone ones. The extensive tests and the experiments in simulation show the ability of the method to solve the real-world sorting problem using multiple mobile manipulators.

==> conclusion.tex <==
We present a planning algorithm for sorting arbitrarily positioned set of objects by their types and predefined orders utilizing multiple mobile manipulators. We have developed four different variations of the proposed algorithms by search strategies, and they all are shown to be complete, two of which are shown to produce feasible solutions for robots to execute fast enough to be used in real world as well. With this work as a baseline, we would develop further by generalizing object geometry. Also, we seek to extend our work beyond stacking applications.\textbf{}
